Adversarial Inter-Group Link Injection Degrades the Fairness of Graph Neural Networks

We present evidence for the existence and effectiveness of adversarial attacks on graph neural networks (GNNs) that aim to degrade fairness. These attacks can disadvantage a particular subgroup of nodes in GNN-based node classification, where nodes of the underlying network have sensitive attributes, such as race or gender. We conduct qualitative and experimental analyses explaining how adversarial link injection impairs the fairness of GNN predictions. For example, an attacker can compromise the fairness of GNN-based node classification by injecting adversarial links between nodes belonging to opposite subgroups and opposite class labels. Our experiments on empirical datasets demonstrate that adversarial fairness attacks can significantly degrade the fairness of GNN predictions (attacks are effective) with a low perturbation rate (attacks are efficient) and without a significant drop in accuracy (attacks are deceptive). This work demonstrates the vulnerability of GNN models to adversarial fairness attacks. We hope our findings raise awareness about this issue in our community and lay a foundation for the future development of GNN models that are more robust to such attacks.

==> Sections/04_attack_model_backup.tex <==

\section{Approach}
% In our work, we aim to build adversarial attacks that aim at reducing the fairness of GNNs.
% First, we introduce the problem of fairness attacks on GNNs.
In this section, we present and analyze a Fairness Attack on GNNs (FA-GNN) that aims at degrading the fairness of GNNs for binary node classification.
We first describe the settings of this attack and explain the attack strategy.
Then we provide a qualitative analysis of the consequences of this fairness attack.
Finally, we illustrate these consequences on synthetic graphs as a proof of concept.
% First we conduct qualitative analysis of four adversarial linking strategies and their effect on statistical parity in node classification.
% We then simulate these linking strategies on synthetic datasets to build intuitions.
% Finally, we formally introduce the attack algorithm.



\subsection{Fairness attack on GNNs}
\label{sec:formulation}
% Building on the  above analysis, 
%and the simulation above,
% We formally introduce Fairness Attacks on GNNs (FA-GNN).
% Here we explain the overall goal of fairness attacks, and define an example of a fairness attack on GNNs (which we name FA-GNN) that adds adversarial edges to the network.
% \hussain{problem: the goal is shared among any attacker on fairness, the restrictions only apply to our instance (FA-GNN).}
% % We consider an adversarial attack with the goal of degrading GNN fairness.
% % First, we describe the overall goal of fairness attacks on GNNs.
% % Then we introduce an example of a fairness attack on GNNs (FA-GNN) by defining the attacker's capabilities and the attack algorithm.
% % We introduce the problem of fairness attack on GNNs by describing the attacker's goal,
% We introduce fairness attacks on GNNs (FA-GNNs) by defining the attacker's goal and capabilities, as well as the attack algorithm.

% 1. we introduce the concept of aagnnf
% 2. we specify the settings and task (node classification, binary attributes, add only edges)
% 3. we describe how we achieve a fagnn given these settings (surrogate GCN)
%3a. how we measure the success of the attack

% First, we introduce the concept of adversarial attacks on the fairness of GNN-based node classification.
% Then we describe the attacker's capabilities and goals that we consider in our paper.
% To provide evidence of such attacks, we construct an adversarial attack on GNN-based binary node classification.
% To that end, we specify the attacker's goal and restrictions, and describe attack strategies to degrade GNNs fairness.

% \para{Attacker's goal.} % \hussain{is this needed anymore?}
The purpose of attacks on GNNs for node classification is typically to decrease the prediction accuracy.
In contrast, attacks on GNNs' fairness aim to degrade the prediction fairness of a \underline{victim GNN} binary node classifier.
The success of the attack can thereby be measured by several fairness metrics~\cite{verma2018fairness}.
\san{I think it makes more sense to start with what the goal of the attacker is in our case and then say that it is in contrast with a typical adversarial setting where the aim is to attack accuracy. Also you use the term victim model for the first time here. I think you should explain the terminology.}

%, which might also guide the attacker's strategy.
%Hence a successful attack needs to take the target fairness measure into consideration.
%, we use  the metrics introduced in Section~\ref{preliminaries}.
% We refer to the target of the attack as the \underline{victim GNN}.
% Degrading fairness can be measured by several popular fairness metrics~\cite{}.
%\para{Settings.}
% \para{Attacker's goal.}
% We consider the case of binary node classification and binary sensitive attributes.
% The attacker's goal is to degrade the prediction fairness of a \underline{victim GNN} binary node classifier.


\para{Attacker's capabilities.}
The data available to the attacker include the structural information, feature information and sensitive attributes of the entire graph as well as the ground-truth classes of some nodes $W \subseteq V$, that is $(V,E,X,y(W),s)$.
% The data available to the attacker include the structural information of the entire network as well as features and sensitive attribute information of all the nodes in the network. However, the ground truth class labels are only available for only a subset of nodes. 
The attacker has the capability of adding edges anywhere in the graph up to a budget, defined by a perturbation rate $\delta > 0$. 
For a perturbation rate $\delta$, the attacker can add up to $\delta |E|$ edges to the graph.
The attacker has no access to the parameters or hyperparameters of the victim GNN model.\meng{the last sentence is about attacker's knowledge, does it make sense to move it along with the first sentence? -->1) knowledge 2) capability}
%Given the extent of knowledge that the attacker possesses, they can design the best possible attack, simulating a worst case scenario for the defender.

\subsection{Attack strategy}
\label{sec:strategy}

We introduce our strategy for a fairness attack on GNNs, that we name FA-GNN.
Similar to~\cite{zugner2018adversarial, zugner2019adversarial}, FA-GNN uses a \underline{surrogate GCN}~\cite{kipf2016semi} model to predict labels for the unlabeled nodes, which makes our attack a grey-box attack~\cite{jin2020adversarial}.
We denote the predictions of the surrogate GCN as $\bar{y}$ to distinguish them from the predictions of the victim GNN $\hat{y}$.
% \meng{1) "they" refer to attacker --> attackers? 2) would it be better if we remove "perhaps"}  \hussain{I would keep they as it is}
% Following the taxonomy from~\cite{jin2020adversarial}, this attack is a poisoning global grey-box attack on GNNs which operates by adding adversarial edges to the graph.

% \para{Attacker's goal.}
% We differentiate between two possible aims of the attacker, assuming (w.l.o.g.) that prediction $\hat{y}=1$ is favorable.
% The attacker's goal is either 1) to disadvantage group $s_0$ by decreasing $SPD$, or 2) to disadvantage group $s_1$ by increasing $SPD$.
% \hussain{absolute anyway}


% This generalization suggests that using the same attack strategy on more than two subsets can be contradictory.
% For example, using DD between $y_1s_1$ and $y_0s_0$ yields opposite results to DD between $y_0s_1$ and $y_1s_0$.
% We do not discuss cases where one attack strategy involves more than two subsets as some combinations contradict each other.
% \para{Choosing the target subset.}
% \hussain{to favor $s_0$ we either use DD on $y_1s_1$ (equiv. to DD on $y_0s_0$) or EE on either $y_0s_1$ or $y_1s_0$. To favor $s_0$ we either use DD on $y_1s_0$ (equiv. to DD on $y_0s_1$) or EE on either $y_0s_0$ or $y_1s_1$ (maybe in the previous subsec)}
% \hussain{since we show a `target' we should be careful and say that EE puts the target at an advantage while DD puts the target at a disadvantage (conclude this subsec like this)}

% \para{Adversarial linking strategies} \label{linking-strategies}
% For a specific subset $a \in \mathcal{S}$, we consider the four naive linking strategies (illustrated in Figure~\ref{fig:linking}).
% Each strategy adds links between random nodes from $a$ and random nodes from a subset with:

\para{Attack algorithm.}
An instance of FA-GNN involves subsets $a,b \in \mathcal{S}=\{y_0s_0,y_0s_1,y_1s_0,y_1s_1\}$ (attacks on more than two subsets can be seen as compositions of attacks on pairs of subsets).
FA-GNN adds links between random nodes from~$a$ and random nodes from~$b$ up to perturbation rate $\delta$ as follows.
\begin{description}
    % \item[Parameters:] a perturbation rate $\delta$ and two subsets $a,b \in \mathcal{S}$.
    % \meng{1) does it make sense to merge "parameters" into "input"? 2) we don't have the subsets yet at the beginning(subset-->subset names?) 3) considering we should first know the strategy then decide subset name $a,b$, a rephrased alternative is below}
    \item[Input:] a clean graph $(V,E,X,y({W}),s)$.
    \item[Label propagation:] train a surrogate GCN model to predict the labels for unlabeled nodes $\bar{y}(V \setminus W)$.\meng{"Label propagation" may refer to another algorithm, I would prefer "Training surrogate" or "Obtaining labels"}
    \item[Building subsets:] combine the sensitive attribute $s$ with known labels $y({W})$ and predictions $\bar{y}(V \setminus W)$ to build subsets ($y_is_j$).
    This determines which nodes belong to $a$ and $b$.
    \item[Add\meng{ing} links:] add $\lfloor\delta |E|\rfloor$ links between random nodes from $a$ and $b$.\meng{or remove all -ing from the steps} 
\end{description}
Choosing $a,b$ reduces to one of the following four linking strategies (illustrated in Figure~\ref{fig:linking} - Top) that connect nodes of
\begin{enumerate}
    \item[(DD)] \emph{D}ifferent class and \emph{D}ifferent group,
    \item[(DE)] \emph{D}ifferent class and \emph{E}qual group,
    \item[(ED)] \emph{E}qual class and \emph{D}ifferent group, or
    \item[(EE)] \emph{E}qual class and \emph{E}qual group, that is $a=b$.
\end{enumerate}

% \iffalse
------------------

\meng{an alternative:}
\para{Attack algorithm.}
An instance of FA-GNN involves subsets $a,b \in \mathcal{S}$ (attacks on more than two subsets can be seen as compositions of attacks on pairs of subsets). Based on the difference of label $y$ and sensitive attribute $s$ in $a,b$, we propose the attack strategy $\rho$ which maps to one of the following four linking strategies (illustrated in Figure~\ref{fig:linking} - Top) that connect nodes of
\begin{enumerate}
    \item[(DD)] \emph{D}ifferent class and \emph{D}ifferent group,
    \item[(DE)] \emph{D}ifferent class and \emph{E}qual group,
    \item[(ED)] \emph{E}qual class and \emph{D}ifferent group, or
    \item[(EE)] \emph{E}qual class and \emph{E}qual group, that is $a=b$.
\end{enumerate}
Each strategy adds links between random nodes from~$a$ and random nodes from~$b$.
The attack works as follows.
\begin{description}
    % \item[Parameters:] a perturbation rate $\delta$ and two subsets $a,b \in \mathcal{S}$.
    \item[Input:] a clean graph $(V,E,X,y({W}),s)$, a perturbation rate $\delta$, the attack strategy $\rho$.
    \item[Label propagation:] train a surrogate GCN model to predict the labels for unlabeled nodes $\bar{y}(V \setminus W)$, combine known labels $y({W})$ with predictions $\bar{y}(V \setminus W)$ to obtain label set $y$.
    \item[Building subsets:] combine the label set $y$ with the sensitive attribute set $s$ to build subsets ($y_is_j$). For strategy $ \rho$, determine target subsets $a$ and $b$.
    \item[Add links:] add $\lfloor\delta |E|\rfloor$ links between random nodes from $a$ and $b$.
\end{description}

-----------------
% \fi

Note that we demonstrate one way of performing a fairness attack via adding edges in this paper, and we leave other types of structural attacks on fairness for future work.
% Note that removing and rewiring edges are also viable options for a structural attack, and that adding edges demonstrates one way of performing a fairness attack.



\subsection{Consequences of fairness attacks}
\label{sec:theoretical-analysis}
We explore the impact of a FA-GNN on the overall statistical parity difference $SPD$ through the following qualitative analysis.
% We use a signed version to denote the parity in favor of nodes with $s=0$.
% \begin{equation}
% \label{eq:signed-parity}
%     SPD = P(\hat{y} = 1 | s = 0) - P(\hat{y} = 1 | s = 1).
% \end{equation}
% In other words, a positive $SPD$ indicates a higher probability that nodes with $s=0$ get the positive class $y=1$, and vice versa.
We can rewrite the formula of Equation~\ref{eq:signed-parity} to adapt to our defined subsets.
\begin{equation}
\begin{split}
    SPD & = P(\hat{y} = 1, y = 0 | s = 0) + P(\hat{y} = 1, y = 1 | s = 0)\\
    & - P(\hat{y} = 1, y = 0 | s = 1) - P(\hat{y} = 1, y = 1 | s = 1).
\end{split}
\end{equation}
We can further reformulate it in terms of statistical measures of the binary classification confusion matrix in (Table~\ref{tab:confusion-matrix})
% In terms of the binary classification confusion matrix (Table~\ref{tab:confusion-matrix}), we can rewrite the formula as
% \begin{equation}
%     SPD = \frac{FP_{s_0}+TP_{s_0}}{n_{s_0}} - \frac{FP_{s_1}+TP_{s_1}}{n_{s_1}},
% \end{equation}
% where $TP_{s=j}$ and $FP_{s=j}$ are the true and false positive counts in group $s=j$ respectively.
% Let's rewrite that in terms of false positives and false negatives (error terms) only.
\begin{equation}
\begin{split}
    SPD &= \frac{FP_{s_0}+TP_{s_0}}{n_{s_0}} - \frac{FP_{s_1}+TP_{s_1}}{n_{s_1}},\\
\end{split} 
\end{equation}
where $FP_{s_j}$ and $TP_{s_j}$ represent the false and true positives counts in group $s=j$, respectively.
We can rewrite that using empirical error terms only
\begin{equation}
\label{eq:sp-confusion}
\begin{split}
    % SPD &= \frac{FP_{s_0}+(n_{y_1s_0}-FN_{s_0})}{n_{s_0}} - \frac{FP_{s_1}+(n_{y_1s_0}-FN_{s_1})}{n_{s_1}}\\
    SPD &= \frac{FP_{s_0}-FN_{s_0}}{n_{s_0}} - \frac{FP_{s_1}-FN_{s_1}}{n_{s_1}} + \frac{n_{y_1s_0}}{n_{s_0}}-\frac{n_{y_1s_1}}{n_{s_1}},
\end{split}
\end{equation}
where $FN_{s=j}$ and $FP_{s=j}$ are the false negative and false positive counts in group $s=j$, respectively.
If we consider a random classifier or a constant classifier, terms in Equation~\ref{eq:sp-confusion} cancel out and $SPD = 0$.
If we consider a perfect classifier, all error terms vanish in Equation~\ref{eq:sp-confusion}, and we get $SPD = n_{y_1s_0}/n_{s_0}-n_{y_1s_1}/n_{s_1}$.
In other words, a perfect predictor is as fair as the original label distribution.
Next, we discuss more practical cases.

\para{Intuition.}
Let us consider any of FA-GNN's linking strategies (Section~\ref{sec:strategy}).
% \dhe{we need to explain why only attack on two subsets. we could argue that more complex attacks that add links between arbitrary number of subsets will be a composition of simpler two subset attacks.}.
%We consider up to two subsets as more complex attacks that add links between an arbitrary number of subsets will be a composition of simpler two subset attacks. \hussain{@Denis, maybe as simple as that?}
% \dhe{i rephrased it a bit. if you agree, just delete this comment.}
Research on GNN attacks suggests that linking nodes of different classes increases the victim GNN's prediction error~\cite{zhang2020gnnguard}.
Depending on this, we assume that linking two subsets of different classes results in higher error rates (more false positives/negatives) on both subsets.
Conversely, we assume that linking nodes from two subsets of the same (equal) class results in lower error rates on both subsets.
Note that these assumptions can mainly hold for homophilic graphs (i.e., where likes attract).
Since classical GNNs are commonly deployed on homophilic graphs~\cite{zhu2020beyond}, we use these assumptions in the main body of the paper.
We explore less practical scenarios (such as heterophilic and random graphs) in Appendix~\ref{app:theory} along with experimental illustration on synthetic data.

After performing the attack on the given graph, we get a new statistical parity difference $SPD' = SPD + \Delta SPD$.
We denote the change in the number of false positives and false negatives on $s_j$ as $\Delta FP_{s_j}$ and $\Delta FN_{s_j}$, respectively.
We neglect the changes of errors on subsets untargeted by the attack, since directly attacked nodes usually exhibit higher error~\cite{zugner2018adversarial}.


\para{Analysis.}
With the above assumptions, we perform an approximate analysis of statistical parity difference.
% Without loss of generality, we discuss linking nodes in $y_1s_1$ the adversarial linking strategy of FA-GNN.
Without loss of generality, we discuss the adversarial linking strategies of FA-GNN from the perspective of nodes in $a = y_1s_1$.



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[b]
\caption{Binary classification confusion matrix with a binary sensitive attribute.}
\label{tab:confusion-matrix}
\small
\begin{tabular}{ll|ll|ll}
                            & Group                 & \multicolumn{2}{c|}{$s=0$}                             & \multicolumn{2}{c}{$s=1$}                             \\
                            & Class                 & \multicolumn{1}{c}{$y=0$} & \multicolumn{1}{c|}{$y=1$} & \multicolumn{1}{c}{$y=0$} & \multicolumn{1}{c}{$y=1$} \\ \hline
\multirow{2}{*}{Prediction} & $\hat{y}=0$           & $TN_{s_0}$                & $FN_{s_0}$                 & $TN_{s_1}$                & $FN_{s_1}$                \\
                            & $\hat{y}=1$           & $FP_{s_0}$                & $TP_{s_0}$                 & $FP_{s_1}$                & $TP_{s_1}$                \\ \hline
                      & \multicolumn{1}{c|}{$\sum$} & $n_{y_0s_0}$              & $n_{y_1s_0}$               & $n_{y_0s_1}$              & $n_{y_1s_1}$              \\ \hline
                  & \multicolumn{1}{c|}{$\sum$} & \multicolumn{2}{c|}{$n_{s_0}$}                         & \multicolumn{2}{c}{$n_{s_1}$}                        
\end{tabular}
\end{table}

    \paragraph{Case $b = y_0s_0$ (DD):} In this case we link nodes from different classes, so following the intuition above, we assume error rates to increase
    $$\Delta FP_{s_0} \geq 0, \Delta FN_{s_1} \geq 0, \Delta SPD = \frac{\Delta FP_{s_0}}{n_{s_0}}+\frac{\Delta FN_{s_1}}{n_{s_1}}\geq 0$$
    We therefore expect that this linking results in an \emph{attack against group $s_1$}.
    Notice that we neglect $\Delta FP_{s_1}$ and $\Delta FN_{s_0}$ since they are not directly affected by the attack.
    We continue the following cases with the same manner.
    \paragraph{Case $b = y_0s_1$ (DE):} Here we also link nodes from different classes, so we assume the error rates to increase
    $$\Delta FP_{s_1} \geq 0, \Delta FN_{s_1} \geq 0, \Delta SPD = \frac{\Delta FN_{s_1}-\Delta FP_{s_1}}{n_{s_1}}$$
    The sign of $\Delta SPD$ depends on the values of $\Delta FN_{s_1}$ and $\Delta FP_{s_1}$.
    This linking results in a change on $SPD$ but the direction is not predictable, so the \emph{attack is not targeted}, that is, it does not specifically increase or decrease $SPD$.
    \paragraph{Case $b = y_1s_0$ (ED):} We link nodes from the same class. Again, following the intuition, we assume error rates to decrease
    $$\Delta FN_{s_0} \leq 0, \Delta FN_{s_1} \leq 0, \Delta SPD = \frac{\Delta FN_{s_1}}{n_{s_1}}-\frac{\Delta FN_{s_0}}{n_{s_0}}$$
    The sign of $\Delta SPD$ is also unpredictable, so the \emph{attack is not targeted} as well.
    If we consider that the error on the clean graph is low, then this attack will not be effective either, as $\Delta FN_{s_0}$ and $ \Delta FN_{s_1}$ will be small.
    \paragraph{Case $b = y_1s_1$ (EE):} Here we also link nodes from the same class, so we assume the error rates to decrease
    $$\Delta FN_{s_1} \leq 0, \Delta SPD = \frac{\Delta FN_{s_1}}{n_{s_1}} \leq 0$$
    We expect this linking to result in an \emph{attack in favor of group $s_1$}.

In conclusion, we expect that linking $y_1s_1$ and $y_0s_0$ (nodes from different classes and different groups, that is DD) results in an attack targeted against $s_1$.
Besides, increasing the intra-connectivity of $y_1s_1$ (i.e.,  EE) results in a targeted attack against $s_0$.
EE only manipulates one subset, and this might not be as effective as DD that increases the connectivity between two subsets.
% We now unify these four cases for all subsets through four linking strategies.
%from the perspective of any subset of nodes.

\para{Initial statistical parity difference.}
The initial signed $SPD$ value may also influence the strategy and outcome of the attack.
For example, an attacker can increase or decrease the signed statistical parity difference $SPD$ with the goal of increasing the absolute statistical parity difference $|SPD|$.
We elaborate more on the initial $SPD$ value and the suitable strategies in Section~\ref{sec:attack-outcome}. 

In the next section, we illustrate the implications of adversarial linking strategies on synthetic datasets.

% Now let's consider a structural attack on the graph that adds links between random nodes of two subsets.
% % Research on GNN attacks and defense have suggested that successful attacks tend to connect nodes of opposite labels~\cite{zhang2020gnnguard} and dissimilar nodes~\cite{wu2019adversarial}.
% % Depending on this, we assume that linking two subsets with opposite labels results in higher error rates (more false positives/negatives) on both subsets.
% % Conversely, assume that linking two subsets with the same labels results in lower error rates on both subsets.
% After performing the attack on the given graph, we get a new $SPD' = SPD + \Delta SPD$.
% We denote the change in the number of false positives and false negatives as $\Delta FP$ and $\Delta FN$ respectively.
% We neglect the changes of errors on subsets untargeted by the attack since directly attacked nodes exhibit higher error~\cite{zugner2018adversarial}.
% Without loss of generality, we discuss linking nodes in $y_1s_1$ to nodes in another subset.



% % \begin{description}
% %     \item[Case $y_0s_0$:]
% \underline{\textit{Case $y_0s_0$:}}
%     $$\Delta SPD = \frac{\Delta FP_{s_0}}{n_{s_0}}+\frac{\Delta FN_{s_1}}{n_{s_1}}$$ % in homophilic nets, we expect the error to go up
%     We discuss the situations where (1) the prediction error increases on both subsets, $\Delta FP_{s_0}, \Delta FN_{s_1} > 0 \Rightarrow \Delta SPD > 0$
%     and (2) the prediction error decreases on both subsets, $\Delta FP_{s_0}, \Delta FN_{s_1} < 0 \Rightarrow \Delta SPD < 0$.
%     In both situations, this linking has an impact on $SPD$.
%     In particular, this linking make the neighborhoods of these subsets either become more similar or more distinct depending on the clean graph.
%     We assume that the prediction error increases if these subsets obtain similar neighborhoods, and decrease if the obtain distinct neighborhoods~\cite{ma2021homophily}.
%     Therefore, we leave out the situation where prediction error increases on one subset and decreases on the other.
%     In homophilic graphs (where GNNs are commonly deployed~\cite{ma2021homophily,zhu2020beyond,hussain2021interplay}), the subsets obtain similar neighborhood, so \emph{we can expect SPD to go up}. 
    
% \underline{\textit{Case $y_0s_1$:}}
%     % \item[Case $y_0s_1$:]
%     $$\Delta SPD = \frac{\Delta FN_{s_1}}{n_{s_1}}-\frac{\Delta FP_{s_1}}{n_{s_1}}$$
%     $FP_{s_1}$ and $FN_{s_1}$ are Type I and Type II errors, so reducing one error generally increases the other (and vice versa).
%     Depending on the classifier, we either have $\Delta FN_{s_1} > 0, FP_{s_1} < 0 \Rightarrow \Delta SPD > 0$ or $\Delta FN_{s_1} < 0, FP_{s_1} > 0 \Rightarrow \Delta SPD < 0$.
%     Therefore, we expect this linking to cause \emph{significant change in SPD}, but the sign of the change depends on the classifier's tendency to predict positive or negative class for the respective subsets.
    
% \underline{\textit{Case $y_1s_0$:}}
%     % \item[Case $y_1s_0$:]
%     $$\Delta SPD = \frac{\Delta FN_{s_1}}{n_{s_1}}-\frac{\Delta FN_{s_0}}{n_{s_0}}$$
%     Reducing both false negatives is possible, and it is in the classifier's interest as it reduces the classification loss. This leads to a negligible change in $SPD$.
%     Otherwise (if the classifier tends to predict the negative class on $y_1$), both terms increase $\Delta FN_{s_0} > 0, \Delta FN_{s_1} > 0$. The increase in one term can cancel out some increase in the other leading to a slower change in $SPD$ than we see in Case $y_0s_0$ for example.
%     In both cases, \emph{we expect no significant change in SPD}.
    
% \underline{\textit{Case $y_1s_1$:}}
%     % \item[Case $y_1s_1$:]
%     $$\Delta SPD = \frac{\Delta FN_{s_1}}{n_{s_1}}$$
%     If the classifier achieves better predictions $y_1s_1$, then $\Delta FN_{s_1} < 0 \Rightarrow \Delta SPD < 0$.
%     In case of worse predictions, $\Delta SPD > 0$.
%     In both cases, this linking has an impact on $SPD$.
%     In homophilic graphs in particular, such linking helps in improving the predictions~\cite{zhang2020gnnguard,wu2019adversarial}, so \emph{we expect SPD to go down}.
% % \end{description}
% Due to symmetry, we can unify these four cases for all subsets through the following linking strategies.

% It is possible that the error decreases if the original graph. This might lead to different results.  (In a general case, this might decrease the error) but the difference of SP will be the same, only in a different sign. Will be bounded in the same way

% Please also note that we use the term target to denote the subset we `target' with our linking.
% It is not necessary that the outcome will be unfair for the target subset.
% For example, if the target subset is $y_1s_1$, then the outcome will favor $s_1$ with EE strategy, while it will favor $s_0$ with DD strategy.

% Depending on the original clean graph $G$, with each linking strategy, the two targeted subset can gain either more similar or more distinct neighborhoods.
% The similarity of neighborhoods can enforce similarity of node representations~\cite{ma2021homophily}.
% Therefore, more similar neighborhoods cause more \textit{inseparable node representations}, while a distinct neighborhood cause other subsets to be relatively less separable.



    
\subsection{Illustration}\label{sec:simulation}
We illustrate FA-GNN on synthetic graphs and observe the GNN's response in terms of statistical parity difference ($SPD$).
We consider graphs of $4\,000$ nodes divided equally into four subsets of size $1\,000$, in the order $y_0s_0$, $y_0s_1$, $y_1s_0$, and $y_1s_1$.

\para{Generating node features.}
For each node, we generate $10$ features based on its class membership and $10$ other features based on its group membership.
This results in a feature matrix $X \in \real^{4\,000 \times 20}$, where $X(u,k)$ is the $k$-th feature of node $u$.
For a node $u \in y_is_j$, we sample 10 features from a normal distribution $X(u,k) \sim \mathcal{N}(\mu_{y_i}(k),\sigma^2)$ where $1 \leq k \leq 10$.
We also sample 10 other features from a normal distribution $X(u,k) \sim \mathcal{N}(\mu_{s_j}(k-10),\sigma^2)$ where $11 \leq k \leq 20$.
$\mu_{y_i} \in [-1,+1]^{10}$ and $\mu_{s_j} \in [-1,+1]^{10}$ are two mean vectors sampled independently at random from $[-1,+1]$.
% In particular, we associate class $y_i$ with a random mean vector $\mu_{y_i} \in [-1,+1]^{10}$, and group $s_j$ with another independent random mean vector $\mu_{s_j} \in [-1,+1]^{10}$.
In our settings, we set $\sigma^2 = 0.5$.
Note that this setup does not assume that node features are independent of group memberships.
% \hussain{doesn't this mean that each single feature is independent anyway and we don't even need to call it `multivariate'? maybe just 10 features, each feature $t$ sampled from $\mathcal{N}(\mu_{y_i,t},0.5)$?}

% \dhe{this is hard to understand}

\para{Generating the clean graph.}
To build our graphs, we use the stochastic block model~\cite{holland1983stochastic} (SBM) on the four subsets.
This requires a symmetric density matrix $M \in [0,1]^{4 \times 4}$ as an input.
As classical GNNs are typically deployed on homophilic graphs~\cite{zhu2020beyond,hussain2021interplay}, we follow a setup where the clean graph is homophilic w.r.t. labels.
% We later address graphs with other characteristics (heterophilic and random graphs) in Appendix~\ref{app:theory}. 
% We choose for any node in these graphs to have $8$ neighbors with the same label on average. 
To that end, we set the intra-label edge density to $0.004$ and the inter-label edge density to $0.0016$.
% This results in $8$ neighbors with the same label and $3.2$ neighbors of the opposite label for each node on average.
% We set a lower inter-label edge density ($0.4$ of the intra-label density, hence $0.0016$).  
This preserves an appropriate level of sparsity and homophily in the graph.
Lower intra-label densities would increase the variance in neighborhood sampling. 
%To keep the graph homophilic, we tune the inter-label edge density to be smaller ($0.4$ of the intra-label density, hence $0.0016$).
Besides, lower inter-label densities could result in extreme homophily, which makes the classification task trivial for the GNN model~\cite{zhu2020beyond,ma2021homophily}.

% \dhe{this is even harder to understand}

\para{Generating the perturbed graph.}
We apply the four strategies DD, DE, ED, EE on subset $a = y_1s_1$.
Let subset $b \in \mathcal{S}$ be the other subset to which we connect nodes of $y_1s_1$.
Let $|E|$ be the number of edges in the clean graph, which we sample using SBM as explained above.
For a perturbation rate $\delta$, we add $\delta |E|$ edges between random nodes from $a$ and random nodes from~$b$.
% Notice that this setup simulates an attacker that has access to the labels of all nodes.

% Now, for an attack with a perturbation rate $\delta$, the total added density is $\delta^+ = \frac{\sum_{i,j}{M_{i,j}}}{2 \times \delta}$.
% Thus, we replace $M'_{a,b} = M'_{b,a} := M_{a,b} + \delta^+$ in the stochastic block matrix.
% Other than indices $a,b$ and $b,a$, $M'_{i,j} := M_{i,j}$.
% We sample the perturbed graph from using SBM with $M'$ as an input stochastic block matrix. \hussain{update this}


\para{Evaluation.} 
After building the graph, we train a graph convolutional network~\cite{kipf2016semi} (GCN) model on the node classification task.
For the training process, we randomly sample $|V_l| = 20$ nodes to be in the training set, while the rest of the nodes are in the test set.
We repeat each trial for $100$ independent runs, implying a different graph structure, node features and GCN weight initialization in each run. 



\begin{figure}
    \begin{flushright}
    \includegraphics[width=.9\linewidth]{Figures/linking-new.png}
    \end{flushright}
    \centering
    \includegraphics[width=\linewidth]{Figures/synth-results.pdf}
    \caption{(Top) Linking strategies involving nodes with $y=1,s=1$.
    Each figure of four circles illustrates a linking strategy.
    Each circle $y_is_j$ represents the subset of all nodes with $y=i,s=j$.
    % Each node with  $y=i,s=j$ belongs to a subset $y_is_j$ (one circle in this figure).
    % We see the four subsets of nodes, with links between with initial links between them in black.
    The green line between two subsets means that the respective strategy adds links between random nodes of these subsets.
    (Bottom) Fairness attacks on synthetic graphs. % Statistical parity on synthetic datasets.
    Each figure shows the $SPD$ of a linking strategy with an increasing perturbation rate on synthetic graphs.
    We see that DD strategy increases $SPD$ and EE strategy reduces $SPD$.
    Meanwhile, ED fluctuates around 0, and DE also fluctuates around 0 with a high variance.
    This shows that, in our simulation, DD and EE degrade the GNN fairness, while DE is inconsistent and ED is ineffective.}
    \label{fig:linking}
\end{figure}
% \begin{figure}
%     \centering
%     \label{fig:synth-results}
% \end{figure}
\para{Results.}
% Here we show the results on the synthetic data and explain that they confirm our theoretical analysis.
We report the statistical parity difference after training the GCN for each strategy across varying perturbation rates $\delta$ between $0.05$ and $0.3$ with steps of $0.025$ (Figure~\ref{fig:linking} - Bottom).
Supporting our qualitative analysis, 
\begin{enumerate*}[label=(\arabic*)]
  \item DD strategy increases $SPD$,
  \item DE strategy fluctuates around $0$,
  \item ED strategy also fluctuates around $0$ without a significant influence on $SPD$ and
  \item EE strategy decreases $SPD$ but at a lower rate than DD.
\end{enumerate*}
Another interesting observation is that DD strategy reaches a peak and then drops with more perturbations.
One hypothesis is that the subsets $y_0s_0$ and $y_1s_1$ are approaching extreme heterophily, which can cause GNNs to achieve lower error rates according to recent research~\cite{ma2021homophily} (note that $\delta=.3$ represents a remarkably high perturbation rate). 
% While such scenarios are well-discussed in~\cite{ma2021homophily}, we focus on the initial parity decrease with lower perturbation rates, and leave this question open for future work.
For a deeper understanding, we also report the changes in error rates from Eq.~(\ref{eq:sp-confusion}) in our experiment in Appendix~\ref{app:error}.
% In these experiments, we set the clean graph to be homophilic.
% We also show the results where the clean graph is heterophilic in Appendix~\ref{app:theory}.
In the following section, we evaluate fairness attacks on real-world data.
